"The Diagram is like Guardrails": Structuring GenAI-assisted Hypotheses Exploration with an Interactive Shared Representation

Data analysis encompasses a spectrum of tasks, from high-level conceptual reasoning to lower-level execution. While AI-powered tools increasingly support execution tasks, there remains a need for intelligent assistance in conceptual tasks. This paper investigates the design of an ordered node-link tree interface augmented with AI-generated information hints and visualizations, as a potential shared representation for hypothesis exploration. Through a design probe (n=22), participants generated diagrams averaging 21.82 hypotheses. Our findings showed that the node-link diagram acts as "guardrails" for hypothesis exploration, facilitating structured workflows, providing comprehensive overviews, and enabling efficient backtracking. The AI-generated information hints, particularly visualizations, aided users in transforming abstract ideas into data-backed concepts while reducing cognitive load. We further discuss how node-link diagrams can support both parallel exploration and iterative refinement in hypothesis formulation, potentially enhancing the breadth and depth of human-AI collaborative data analysis.

==> cutting-room-floor/4-results-1.tex <==
\section{Results}
\label{sec:results}

\subsection{Summary of Participant Interactions with Tool}
\label{res:overview}

% The hypothesis exploration tool received a predominantly positive reception from participants, as evidenced by responses to Q5 in our semi-structured interview. A majority (82\%) expressed enthusiasm, exemplified by P12's statement: ``I absolutely would use this, 100\%." One participant (9\%) showed selective interest, expressing openness to the tool's data visualization capabilities while reserving judgment on its use for hypothesis formulation. The final participant (9\%) cited a commitment to originality and privacy concerns: ``I'm trying to make something novel myself. I don't want to have to cite it or accidentally give away one of my ideas." 


To contextualize our analysis of how our system's shared representation and information hint designs impacted hypothesis exploration, we first describe overall quantitative trends in participants' interactions with the tool. We analyzed the node-link diagram structures generated during the study. On average, diagrams contained 21.82 nodes ($std = 8.78$), reached a maximum depth of 3.86 levels ($std = 1.32$), and had a maximum breadth of 8.09 ($std = 3.06$). To account for the actual number of nodes explored by each participant, rather than just the number of nodes created, we tracked two actions: clicking existing nodes and generating new hypotheses. As illustrated in Figure \ref{fig:nodes-count}, participants clicked nodes an average of 31.41 times ($std = 17.17$) and generated new hypotheses 4.95 times ($std = 2.72$). In total, participants explored nodes an average of 36.36 times ($std = 18.89$). Additionally, we examined user engagement with AI-generated visualizations corresponding to each hypothesis, with Figure \ref{fig:engage-hist} depicting the frequency of initial expansions and re-expansions of these visual hypotheses. We also present examples of AI-generated hypotheses that the first five participants bookmarked in Table \ref{tab:hypotheses}. These examples illustrate how the generated hypotheses went beyond simple pairwise correlation predictions, and incorporated more complex and nuanced ideas such as ``compounding effect." This was particularly the case for hypotheses at deeper levels of the exploration tree.

Considering the interview results, the hypothesis exploration tool received a predominantly positive reception from participants as evidenced by responses to Q5 in the interview. A majority (20/22) expressed enthusiasm, exemplified by P12's statement: ``I absolutely would use this, 100\%." One participant showed selective interest, expressing openness to the tool's data visualization capabilities while reserving judgment on its use for hypothesis formulation. Another participant cited a commitment to originality and privacy concerns: ``I'm trying to make something novel myself. I don't want to have to cite it or accidentally give away one of my ideas."

\begin{table}
\centering
\begin{tabular}{|p{0.02\textwidth}|p{0.16\textwidth}|p{0.65\textwidth}|p{0.05\textwidth}|}
\hline
\textbf{ID} & \textbf{Hypothesis} & \textbf{Description} & \textbf{Level}\\
\hline
P1 & Age Effect & There is a variance in income between married and non-married individuals within different age groups. & 3 \\
\hline
P2 & Occupation Type & There is a significant difference in income levels based on occupation types between married and unmarried individuals. & 2 \\
\hline
P2 & Gender Impact & There is a significant correlation between holding an advanced degree and higher incomes with the additional factor of gender, affecting married individuals differently compared to unmarried individuals. & 4 \\
\hline
P3 & Community Integration & There is a stronger positive correlation between Ivy League education and higher lifetime income for underrepresented racial groups in highly integrated communities. & 4 \\
\hline
P4 & Experience Amplifier & There is a \textbf{compounding effect} of work experience on income, which is amplified with each additional degree. & 2 \\
\hline
P5 & Investment Growth & Higher income earners exhibit a faster growth rate of their financial assets over time. & 5 \\
\hline
\end{tabular}
\caption{AI-generated Hypotheses Bookmarked by Participant 1-5.}
\label{tab:hypotheses}
\end{table}

\begin{figure}
\includegraphics[width=1.\textwidth]{figures/Node-count.png}
  \caption{Count of nodes by level, starting from level 2 given that level 0 always has 1 analysis intent node and level 1 always has 5 initial hypothesis nodes. As the depth increases, the count of nodes per level progressively decreases, reflecting a more focused analysis at deeper levels of the tree structure.}
  \Description{}
  \label{fig:node-count-by-level}
\end{figure}


\begin{figure}
\includegraphics[width=1\textwidth]{figures/Counts.png}
  \caption{Counts of total number of nodes explored (number of nodes clicked + number of new hypothesis branch generated, a new node will be displayed when a new branch is generated), number of nodes clicked, number of new hypothesis branch generated.}
  \Description{}
  \label{fig:nodes-count}
\end{figure}

\begin{figure}
\includegraphics[width=1\textwidth]{figures/Engage.png}
  \caption{Histograms depicting user engagement with visual hypotheses. The data illustrates two types of interactions: initial expansion (opening a visual hypothesis for the first time) and re-expansion (reopening a previously viewed visual hypothesis). Light blue bars represent participants who did not (re-)expand any visual hypothesis. The breakdown for each participant can be found in Table \ref{tab:engagement} in Appendix \ref{appendix:B}.}
  \Description{}
  \label{fig:engage-hist}
\end{figure}

\begin{figure}
\includegraphics[width=1\textwidth]{figures/Backtrack.png}
  \caption{Histograms depicting backtrack behaviors: backtracking previously created branches. The data illustrates three types of backtrack behaviors: high level backtrack and generate, high level backtrack only, and other backtrack instances. The breakdown for each participant can be found in Table \ref{tab:backtrack} in Appendix \ref{appendix:C}.}
  \Description{}
  \label{fig:backtrack-hist}
\end{figure}

The exploration process exhibited complex patterns, exemplified by the backtracking behaviors of P3 (Figure \ref{fig:teaser} and Figure \ref{fig:P3} in Appendix \ref{appendix:B}). P3's process, which included 17 instances of backtracking, prompted a more comprehensive analysis of this behavior across all participants. Figure \ref{fig:backtrack-hist} illustrates various types of backtracking behaviors, including \textit{high level backtrack and generate} (revisit a hypothesis node on a higher level and not on the trajectory from the current node to the root node, and generate new branch from the node), \textit{high level backtrack only} (only revisit a hypothesis node on a high level and not on the current trajectory) and \textit{other backtrack} instances (revisit a hypothesis node but not on a higher level). Besides, four participants chose to regenerate and replace previous branches, with three doing so without backtracking and one employing other backtracking methods.

\begin{figure}
\includegraphics[width=0.8\textwidth]{figures/Hypo-iteration.png}
  \caption{Example of hypothesis iteration from P10.}
  \Description{}
  \label{fig:hypo-iteration}
\end{figure}

\subsection{Ordered Node-link Diagram as Shared Representation of Analysis Pathways}

The semi-structured interview results revealed that the ordered node-link diagram could serve as an effective shared representation for hypothesis exploration by providing a structured workflow, supporting overview and backtracking capabilities, and facilitating rapid prototyping of alternative hypotheses.

\subsubsection{Structured Workflow and Focused Exploration}

While the diagram supported broad exploration, it also provided a structured framework that some users likened to ``guardrails". This structure helped focus users' thinking without overly constraining their creativity. A developer (P10) described this balance:

\begin{quote}
``\textbf{The tree diagram is like guardrails} I would say yes it does (help me), because it limits my imagination down to kind of selectable options. So it puts boundaries on my creativity [while] still allowing me to, like, follow different paths I might have, that I might come up with. So like guardrails I guess would probably be the best way to sum it up. \textbf{The guardrails it imposes focuses me}." (P10, Developer, Figure \ref{fig:hypo-iteration})
\end{quote}

The tree-like structure of the diagram also facilitated a clear workflow for drilling down into specific hypotheses. Users appreciated how it organized ideas into ``buckets" and allowed for systematic exploration:

\begin{quote}
``I think it's really helpful because it puts like the hypothesis into \textbf{buckets}. So you know that you will have a hypothesis for location level, a hypothesis for the work hours. And at the end, I think that this advantage of that tree diagram could be that \textbf{you only focus on one topic and forget about the rest}." (P19, Data scientist)
\end{quote}

\begin{quote}
``It is really helpful in connecting from one hypothesis to another hypothesis until it achieves my goal, right? That is the best part of [the] tree diagram, that helped me to drive through each and every hypothesis at each level and \textbf{drill down to my goal}. That is the best part of this tree, this hypothesis model." (P13, Consultant)
\end{quote}

Participants found the logical flow and visual organization of the diagram conducive to comprehending AI-generated multi-thread hypotheses:

\begin{quote}
``It just gives you a \textbf{logical flow} [..] like, which variables belong in which. It's like a visualization of where variables belong, where they're clustered. Yeah, it just means you go through it very quickly." (P12, UX researcher)
\end{quote}

\begin{quote}
``It allows you to figure out how things are connected. I thought \textbf{it was pretty easy to read and follow}. This helps me understand the data set by helping me understand what different hypothesis were connected and how [and] under [..] what topic." (P3, Global sales, Figure \ref{fig:teaser})
\end{quote}

\begin{quote}
``I mean its user interface is super easy to use. I mean you can click and explore. Uh, and I feel like \textbf{it's very easy to read} because the options are spread out enough. I mean, as the tree gets further down, it gets more specific. So I like that." (P5, Developer, Figure \ref{fig:user-journey})
\end{quote}

\subsubsection{Supporting Overview and Backtracking}

The ordered node-link diagram offered a comprehensive and hierarchically structured visualization of the entire hypothesis space. A key advantage of this overview, as elaborated in Section \ref{res:overview}, was its ability to facilitate backtracking. This feature empowered users to revisit and reconsider earlier hypotheses, enhancing the breadth of their exploration. As one consultant (P18) noted:

\begin{quote}
``This visualization tree, \textbf{it's like [an] organized hierarchy} [..]. It was a structured and where we can easily get to know like, if we miss it somewhere, for example, in the educational level option, if you miss somewhere then to \textbf{recreate} and to \textbf{reread} it. So that time, this hierarchy level tree structure visualization helps us to \textbf{check again}, \textbf{recheck and analyze it}." (P18, Consultant)
\end{quote}

The visual structure also helped users identify areas of focus within their analysis:

\begin{quote}
``It helps to determine \textbf{which area it is more focused}, like which area it is affecting, like for what is the main reason of in income inequality and education level, in which area of education level it's more affecting. What is the main cause of income inequality?" (P9, Developer)
\end{quote}

\subsubsection{Rapidly Prototyping Alternative Hypotheses to Avoid Fixation}

The node-link diagram enabled users to quickly generate and explore multiple hypotheses simultaneously. This multi-threaded prototyping approach was particularly appreciated by participants for its ability to broaden their analytical perspective. As one UX researcher (P12) noted:

\begin{quote}
``What I thought [..] was really cool is every time you've done your piece of analysis, as you go to your supervisor and you say, `Look, this is what I found.' 'Ohh that's really interesting. I wonder if you looked at it this way', but you never have time to do that... So from that point of view, I think \textbf{it's really good for those additional hypothesis} that you might want to go in and test." (P12, UX researcher)
\end{quote}

This sentiment was echoed by other participants, who valued the ability to explore multiple options and dimensions:

\begin{quote}
``When you propose a new hypothesis, \textbf{it does not give you only one option}. It gives you more than one, so you can start like exploring other branches and so that was really helpful." (P19, Data scientist)
\end{quote}

\begin{quote}
``It gives me the options instead of me thinking of it. It gives me the \textbf{multiple options} based on my hypothesis. What I am thinking of right? So that dimension it is giving it for the next level of hypothesis. I want to create it, so that is what the tool is helping us. That is the best part of it. So once I finalize job rule right, then the successive hypothesis, when it creates it gives 3 dimensions right? So one is \textbf{different dimensions}, that is what it is helping us." (P13, Consultant)
\end{quote}

Moreover, parallel prototyping helped users avoid fixation and bias in their analysis. Alternative hypotheses encouraged users to consider variables and relationships they might have otherwise overlooked. Participants recognized this benefit:

\begin{quote}
``I think it is a very useful tool that would help kind of \textbf{take away bias} to a certain extent. I feel like we have a lot of bias or too much personal views that can kind of formulate hypothesis." (P3, Global sales, Figure \ref{fig:teaser})
\end{quote}

\begin{quote}
``And I think as well, like researchers tend to get, tend to get \textbf{dug in with particular variables}, say like if you're if genders on your mind, they'll think of gender, but maybe it won't cross their mind to look at marital status. But when it's there in front of you, you're gonna `Ohh yeah, why don't I think? Let's have a look at that as well'." (P12, UX researcher)
\end{quote}

\begin{quote}
``There was probably \textbf{prior biases}...if you were to ask me like without having seen any of this tool, what do you think correlates to higher income? I probably could have told you years of experience and like number of the degrees." (P4, Business technology)
\end{quote}

\subsubsection{Multi-thread vs Single-thread? Perspectives on Including Chatbot in the Interface}

In Q4 of our semi-structured interviews, we explored participants' views on potentially incorporating a chatbot into the interface. Approximately half of the participants expressed that the existing multi-threaded visualization adequately met their needs for hypothesis exploration and analysis. For example, P8 mentioned the importance of maintaining detailed, structured information flows that the current multi-threaded diagram provides:

\begin{quote}
``\textbf{Chatbot is only end-user oriented}. We (data scientists) need something \textbf{intermediary}... when I go to the manager, he needs the insight only. He doesn't want that full narrative." (P8, Data scientist)
\end{quote}

This quote addresses the divergent needs within the data analysis workflow. Data scientists require intermediary results and detailed analysis paths, which the current multi-threaded visualization provides but a chatbot might not. Conversely, their managers often need only concise, final insights, which could potentially be fulfilled by a chatbot interface. Other participants expressed interests for the inclusion of a chatbot, seeing potential benefits for enhancing the depth of exploration:

\begin{quote}
``I'd like a chatbot. I think it would be nice to be able to talk to the hypothesis as if you were talking to \textbf{someone defending that hypothesis}, because I [..] feel like that's what people do." (P2, Developer, Figure \ref{fig:node-count-by-level})
\end{quote}

\begin{quote}
``Yeah, actually chatting about a hypothesis. Like let's say I get to hear and I wanted to try discussing it. \textbf{Like a debater} at this point that I could then [be] either for or against." (P10, Developer)
\end{quote}

% \subsubsection{Potential Improvements}
% While the ordered node-link diagram was generally well-received, participants suggested several potential improvements:

% \begin{enumerate}
% \item Offering stronger user control over hypothesis exploration, such as the ability to iterate on a single hypothesis or generate more than three hypotheses at a time.
% \item Allowing direct manipulation of dataset columns to generate hypotheses.
% \item Connecting or combining relevant hypotheses and highlighting differences between nodes about the same variables.
% \item Showing branches from one node with different user inputs and labeling each node with user inputs.
% \end{enumerate}

\subsection{AI-generated Multimodal Information Hints for Deciding Analysis Pathway}

The interview results also showed that the AI-generated multimodal information hints played an important role in guiding users to decide on analysis pathways to pursue during hypothesis exploration. This section explores how visual hypotheses served as affirming hints and how the blending of hypotheses and charts reduced context switching effort.

\subsubsection{Visual Hypotheses Enable Judgment of Hypothesis Grounding in Data}
Participants found that the visual hypotheses generated by the system suggested whether there were evidences of their ideas or not. This visual representation helped transform abstract thoughts into data-backed concepts. P4 and P8 described this benefit:

\begin{quote}
``I will say that the visualization of the census data was helpful in \textbf{confirming} the potential income based on the higher degrees. So it was \textbf{affirming} of that. I'm further also just the visual on the working hours and how scattered that was also \textbf{affirmed}." (P4, Business technology)
\end{quote}

\begin{quote}
``It showed me data that was \textbf{reaffirming} to my hypothesis...Like it would just be like an idea of my head that would have had no backing. The fact that I saw it with data is like OK, now this has more credibility. I'm more willing to follow it than I would have if I had just thought of it." (P8, Data scientist)
\end{quote}

The direct nature of visual hypotheses was particularly appreciated. As one researcher (P1) noted, ``I guess most useful part is the figure like the visualization...hypothesis, it's kind of indirect." This sentiment was echoed by a data scientist (P19):

\begin{quote}
``I think it's really really useful because at the end the line charts, the line graph, \textbf{it's really useful to have like a graph that shows or that is directly associated with the hypothesis} that you are seeing...I think having the charts in here, it's really really useful, to really understand what is happening, to be sure that the hypothesis that you are proposing is tied to a graph"
\end{quote}

\subsubsection{Blending Hypotheses and Charts}
An advantage of the multimodality was the seamless integration of hypotheses and visualizations. This feature reduced the effort associated with context switching between hypothesis formulation and chart creation. A data scientist (P8) enthusiastically described this benefit:

\begin{quote}
``It helps me very much and then really we love it. Really. I love it. I can say definitely it helps. The chart and the narrative. And then I get immediately and instantly, which can be transferred visualization I can say because usually we struggle with the visualization and the content when GenAI gives both. It's really easier for us."
\end{quote}

The efficiency gained from this blended approach was widely appreciated. Another data scientist (P19) noted:

\begin{quote}
``I will say that it's really easy to get hypothesis and get like charts that support the hypothesis really quick. So that's an easy way to maybe start exploring data and see what the data has, and go through there, and start like going a little bit more specific."
\end{quote}

% \subsubsection{Providing Supporting Text}
% The inclusion of supporting text as part of the multimodal information hints provided context for users. This feature helped users understand the novelty and relevance of their hypotheses within the broader research landscape. P11 (developer) explained:

% \begin{quote}
% ``It does kind of let you know someone else has come for or done that idea. Like if one we're doing trying to make their own research on something novel, then knowing, you know, at least a quick hey, has someone already tried this or not could help you. Try to test something further or no, maybe no one's thought along this line."
% \end{quote}

% \subsubsection{Potential Improvements}

% While the multimodal information hints were generally well-received, participants suggested several potential improvements. These included providing sources for preliminary results (such as code) and related work (like citations and external links) to enhance the explainability of the outputs. Additionally, participants proposed converting the hypothesis, preliminary results, and related work into preliminary presentation drafts such as slides, which could potentially make the information more accessible and easier to digest.

==> cutting-room-floor/4-results-2.tex <==
\section{Results}
\label{sec:results}

\subsection{Summary of Participant Interactions with Tool}
\label{res:overview}

% The hypothesis exploration tool received a predominantly positive reception from participants, as evidenced by responses to Q5 in our semi-structured interview. A majority (82\%) expressed enthusiasm, exemplified by P12's statement: ``I absolutely would use this, 100\%." One participant (9\%) showed selective interest, expressing openness to the tool's data visualization capabilities while reserving judgment on its use for hypothesis formulation. The final participant (9\%) cited a commitment to originality and privacy concerns: ``I'm trying to make something novel myself. I don't want to have to cite it or accidentally give away one of my ideas." 


% To contextualize our analysis of how our system's shared representation and information hint designs impacted hypothesis exploration, we first describe overall quantitative trends in participants' interactions with the tool. %We analyzed the node-link diagram structures generated during the study. 

Participants explored a substantial number of hypotheses: on average, diagrams contained 21.82 nodes ($std = 8.78$), reached a maximum depth of 3.86 levels ($std = 1.32$), and had a maximum breadth of 8.09 ($std = 3.06$). To account for the actual number of nodes explored by each participant, rather than just the number of nodes created, we tracked two actions: clicking existing nodes and generating new hypotheses. As illustrated in Figure \ref{fig:nodes-count}, participants clicked nodes an average of 31.41 times ($std = 17.17$) and generated new hypotheses 4.95 times ($std = 2.72$). In total, participants explored nodes an average of 36.36 times ($std = 18.89$). Additionally, we examined user engagement with AI-generated visualizations corresponding to each hypothesis, with Figure \ref{fig:engage-hist} depicting the frequency of initial expansions and re-expansions of these visual hypotheses. 

Table \ref{tab:hypotheses} shows representative examples of hypotheses generated by our system during the user study. On average, hypotheses generated by our system appeared to go beyond simple pairwise correlation predictions, incorporating more complex and nuanced ideas: for instance, our system generated a hypothesis that \todo{write this out, including a bit of backstory on how it was generated, what prior context, etc. (labeled ``compounding effect")}. \todo{Hypotheses that were deeper in the diagram's hierarchy were particularly complex and nuanced, illustrating the potential value of the representation as a way for analysts to usefully steer deeper exploration of the hypothesis space.} %To further illustrate the generated hypotheses and the hypothesis exploration and iteration process, we present examples of AI-generated hypotheses bookmarked by the first five participants in Table \ref{tab:hypotheses}. These examples demonstrate how the 

These overall patterns of interaction lead us to believe that participants' had sufficiently substantial interactions with our tool to provide informative reflections on how our system's shared representation and information hint designs relate to the key design goals of balancing breadth and depth, enabling nonlinear exploration, and enabling integrated engagement with data during hypothesis exploration.%, we first describe overall quantitative trends in participants' interactions with the tool. 


% Next, we examine how hypotheses were generated. Specifically, we highlight two types of hypothesis iteration: adding new components and modifying existing components (Figure \ref{fig:hypo-adding}). This iterative conceptual process aligns with prior work \cite{dingFluidTransformersCreative2023}, which describes cycles of conceptual addition, rejection, and modification (rejection and addition).

Based on the interview results for Q5 measuring overall attitudes toward the system, the hypothesis exploration tool received positive feedback from 20 out of 22 participants, such as P12: ``I absolutely would use this, 100\%." One participant expressed selective interest, showing appreciation for the tool's data visualization features but remaining cautious about its utility for hypothesis formulation. Another participant cited a commitment to originality and privacy concerns: ``I'm trying to create something novel myself. I don't want to have to cite it or accidentally reveal one of my ideas."

\begin{table}
\centering
\begin{tabular}{|p{0.02\textwidth}|p{0.16\textwidth}|p{0.65\textwidth}|p{0.05\textwidth}|}
\hline
\textbf{ID} & \textbf{Hypothesis} & \textbf{Description} & \textbf{Level}\\
\hline
P1 & Age Effect & There is a variance in income between married and non-married individuals within different age groups. & 3 \\
\hline
P2 & Occupation Type & There is a significant difference in income levels based on occupation types between married and unmarried individuals. & 2 \\
\hline
P2 & Gender Impact & There is a significant correlation between holding an advanced degree and higher incomes with the additional factor of gender, affecting married individuals differently compared to unmarried individuals. & 4 \\
\hline
P3 & Community Integration & There is a stronger positive correlation between Ivy League education and higher lifetime income for underrepresented racial groups in highly integrated communities. & 4 \\
\hline
P4 & Experience Amplifier & There is a \textbf{compounding effect} of work experience on income, which is amplified with each additional degree. & 2 \\
\hline
P5 & Investment Growth & Higher income earners exhibit a faster growth rate of their financial assets over time. & 5 \\
\hline
\end{tabular}
\caption{AI-generated Hypotheses Bookmarked by Participant 1-5.}
\label{tab:hypotheses}
\end{table}

% \begin{figure}
% \includegraphics[width=1\textwidth]{figures/Hypo-adding.png}
%   \caption{Example of hypothesis iteration by adding new components and modifying existing components from P10.}
%   \Description{}
%   \label{fig:hypo-adding}
% \end{figure}

% \begin{figure}
% \includegraphics[width=1\textwidth]{figures/Hypo-changing.png}
%   \caption{Example of hypothesis iteration by modifying existing components (P1).}
%   \Description{}
%   \label{fig:hypo-changing}
% \end{figure}

\begin{figure}
\includegraphics[width=1.\textwidth]{figures/Node-count.png}
  \caption{Count of nodes by level, starting from level 2 given that level 0 always has 1 analysis intent node and level 1 always has 5 initial hypothesis nodes. As the depth increases, the count of nodes per level progressively decreases, reflecting a more focused analysis at deeper levels of the tree structure.}
  \Description{}
  \label{fig:node-count-by-level}
\end{figure}


\begin{figure}
\includegraphics[width=1\textwidth]{figures/Counts.png}
  \caption{Counts of total number of nodes explored (number of nodes clicked + number of new hypothesis branch generated, a new node will be displayed when a new branch is generated), number of nodes clicked, number of new hypothesis branch generated.}
  \Description{}
  \label{fig:nodes-count}
\end{figure}

\begin{figure}
\includegraphics[width=1\textwidth]{figures/Engage.png}
  \caption{Histograms depicting user engagement with visual hypotheses. The data illustrates two types of interactions: initial expansion (opening a visual hypothesis for the first time) and re-expansion (reopening a previously viewed visual hypothesis). Light blue bars represent participants who did not (re-)expand any visual hypothesis. The breakdown for each participant can be found in Table \ref{tab:engagement} in Appendix \ref{appendix:B}.}
  \Description{}
  \label{fig:engage-hist}
\end{figure}

\begin{figure}
\includegraphics[width=1\textwidth]{figures/Backtrack.png}
  \caption{Histograms depicting backtrack behaviors: backtracking previously created branches. The data illustrates three types of backtrack behaviors: high level backtrack and generate, high level backtrack only, and other backtrack instances. The breakdown for each participant can be found in Table \ref{tab:backtrack} in Appendix \ref{appendix:C}.}
  \Description{}
  \label{fig:backtrack-hist}
\end{figure}

The exploration process exhibited complex patterns, exemplified by the backtracking behaviors of P3 (Figure \ref{fig:teaser} and Figure \ref{fig:P3} in Appendix \ref{appendix:B}). P3's process, which included 17 instances of backtracking, prompted a further analysis of this behavior across all participants. Figure \ref{fig:backtrack-hist} illustrates various types of backtracking behaviors, including \textit{high level backtrack and generate} (revisit a hypothesis node on a higher level and not on the trajectory from the current node to the root node, and generate new branch from the node), \textit{high level backtrack only} (only revisit a hypothesis node on a high level and not on the current trajectory) and \textit{other backtrack} instances (revisit a hypothesis node but not on a higher level).

% Besides, four participants chose to regenerate and replace previous branches, with three doing so without backtracking and one employing other backtracking methods.

\subsection{Design Goal 1: Enable Users to Balance Breadth and Depth of Exploration}

\subsubsection{Structured Workflow and Focused Exploration}

% While the diagram supported broad exploration, users described experiencing it as a structured framework that some users likened to ``guardrails". 
Participants described experiencing the diagram as a structure that helped them focus their thinking without overly constraining their creativity and broad exploration. A developer (P10) evocatively described this experience in terms of helpful ``guardrails'' for exploration:

\begin{quote}
``\textbf{The tree diagram is like guardrails} I would say yes it does (help me), because it limits my imagination down to kind of selectable options. So it puts boundaries on my creativity [while] still allowing me to, like, follow different paths I might have, that I might come up with. So like guardrails I guess would probably be the best way to sum it up. \textbf{The guardrails it imposes focuses me}." (P10, Developer, Figure \ref{fig:hypo-adding})
\end{quote}

Other participants described how they experienced the tree-like structure of the diagram facilitating %a 
% clear workflow for 
drilling down into specific hypotheses without losing sight of the broader exploration. %Users appreciated how it organized ideas into ``buckets" and allowed for systematic exploration. 
For instance, P19 (a data scientist) described how they were able to use the representation to put ``hypothesis into \textbf{buckets}. So you know that you will have a hypothesis for location level, a hypothesis for the work hours. And at the end, I think that this advantage of that tree diagram could be that \textbf{you only focus on one topic and forget about the rest}." Similarly, P13 (a consultant) said, ``[the diagram] is really helpful in connecting from one hypothesis to another hypothesis until it achieves my goal, right? That is the best part of [the] tree diagram, that helped me to drive through each and every hypothesis at each level and \textbf{drill down to my goal}.''

% \begin{quote}
% ``I think it's really helpful because it puts like the hypothesis into \textbf{buckets}. So you know that you will have a hypothesis for location level, a hypothesis for the work hours. And at the end, I think that this advantage of that tree diagram could be that \textbf{you only focus on one topic and forget about the rest}." (P19, Data scientist)
% \end{quote}

% \begin{quote}
% ``It is really helpful in connecting from one hypothesis to another hypothesis until it achieves my goal, right? That is the best part of [the] tree diagram, that helped me to drive through each and every hypothesis at each level and \textbf{drill down to my goal}. That is the best part of this tree, this hypothesis model." (P13, Consultant)
% \end{quote}

Part of this structure appeared to be rooted in the logical flow and visual organization of the diagram, which enabled them to make sense of and keep track of the overall structure of their exploration. P12 (a UX researcher), for example, % conducive to comprehending AI-generated multi-thread hypotheses:
described the experience in this way:
\begin{quote}
``It just gives you a \textbf{logical flow} [..] like, which variables belong in which. It's like a \textbf{visualization of where variables belong, where they're clustered}. Yeah, it just means you go through it very quickly." (P12, UX researcher)
\end{quote}

Similarly, P3 (a global sales \todo{role?}) described how the diagram enabled sensemaking of how the hypotheses were related:
\begin{quote}
``It allows you to figure out how things are connected. I thought it was pretty easy to read and follow. This helps me understand the data set by helping me \textbf{understand what different hypothesis were connected and how [and] under [..] what topic}." (P3, Global sales, Figure \ref{fig:teaser})
\end{quote}

Finally, P5 (a developer) appreciated how the multi-threaded structure was easy to navigate and explore because ``the options are spread out enough...[and] as the tree gets further down, it gets more specific.''

% \begin{quote}
% ``I mean its user interface is super easy to use. I mean you can click and explore. Uh, and I feel like \textbf{it's very easy to read} because the options are spread out enough. I mean, as the tree gets further down, it gets more specific. So I like that." (P5, Developer, Figure \ref{fig:user-journey})
% \end{quote}

\subsubsection{Supporting Overview and Backtracking}

The ordered node-link diagram offered a hierarchically structured visualization of the entire hypothesis space. A key advantage of this overview, as elaborated in Section \ref{res:overview}, was its ability to facilitate backtracking. This feature empowered users to revisit and reconsider earlier hypotheses, enhancing the breadth of their exploration. As one consultant (P18) noted:

\begin{quote}
``This visualization tree, \textbf{it's like [an] organized hierarchy} [..]. It was a structured and where we can easily get to know like, if we miss it somewhere, for example, in the educational level option, if you miss somewhere then to \textbf{recreate} and to \textbf{reread} it. So that time, this hierarchy level tree structure visualization helps us to \textbf{check again}, \textbf{recheck and analyze it}." (P18, Consultant)
\end{quote}

The visual structure also helped users identify areas of focus within their analysis:

\begin{quote}
``It helps to determine \textbf{which area it is more focused}, like which area it is affecting, like for what is the main reason of in income inequality and education level, in which area of education level it's more affecting. What is the main cause of income inequality?" (P9, Developer)
\end{quote}

\subsection{Design Goal 2: Supporting Non-linear Exploration of Hypotheses}

% Ordered Node-link Diagram as Shared Representation of Analysis Pathways

% The semi-structured interview results revealed that the ordered node-link diagram could serve as an effective shared representation for hypothesis exploration by providing a structured workflow, supporting overview and backtracking capabilities, and facilitating rapid prototyping of alternative hypotheses.

\subsubsection{Rapidly Prototyping Alternative Hypotheses to Avoid Fixation}

The node-link diagram enabled users to quickly generate and explore multiple hypotheses simultaneously. This multi-threaded prototyping approach was particularly appreciated by participants for its ability to broaden their analytical perspective. As one UX researcher (P12) noted:

\begin{quote}
``What I thought [..] was really cool is every time you've done your piece of analysis, as you go to your supervisor and you say, `Look, this is what I found.' 'Ohh that's really interesting. I wonder if you looked at it this way', but you never have time to do that... So from that point of view, I think \textbf{it's really good for those additional hypothesis} that you might want to go in and test." (P12, UX researcher)
\end{quote}

This sentiment was echoed by other participants, who valued the ability to explore multiple options and dimensions:

\begin{quote}
``When you propose a new hypothesis, \textbf{it does not give you only one option}. It gives you more than one, so you can start like exploring other branches and so that was really helpful." (P19, Data scientist)
\end{quote}

\begin{quote}
``It gives me the options instead of me thinking of it. It gives me the \textbf{multiple options} based on my hypothesis. What I am thinking of right? So that dimension it is giving it for the next level of hypothesis. I want to create it, so that is what the tool is helping us. That is the best part of it. So once I finalize job rule right, then the successive hypothesis, when it creates it gives 3 dimensions right? So one is \textbf{different dimensions}, that is what it is helping us." (P13, Consultant)
\end{quote}

Moreover, parallel prototyping helped users avoid fixation and bias in their analysis. Alternative hypotheses encouraged users to consider variables and relationships they might have otherwise overlooked. Participants recognized this benefit:

\begin{quote}
``I think it is a very useful tool that would help kind of \textbf{take away bias} to a certain extent. I feel like we have a lot of bias or too much personal views that can kind of formulate hypothesis." (P3, Global sales, Figure \ref{fig:teaser})
\end{quote}

\begin{quote}
``And I think as well, like researchers tend to get, tend to get \textbf{dug in with particular variables}, say like if you're if genders on your mind, they'll think of gender, but maybe it won't cross their mind to look at marital status. But when it's there in front of you, you're gonna `Ohh yeah, why don't I think? Let's have a look at that as well'." (P12, UX researcher)
\end{quote}

\begin{quote}
``There was probably \textbf{prior biases}...if you were to ask me like without having seen any of this tool, what do you think correlates to higher income? I probably could have told you years of experience and like number of the degrees." (P4, Business technology)
\end{quote}

\subsubsection{Multi-thread vs Single-thread? Perspectives on Including Chatbot in the Interface}

In Q4 of our semi-structured interviews, we explored participants' views on potentially incorporating a chatbot into the interface. Approximately half of the participants expressed that the existing multi-threaded visualization adequately met their needs for hypothesis exploration and analysis. For example, P8 mentioned the importance of maintaining detailed, structured information flows that the current multi-threaded diagram provides:

\begin{quote}
``\textbf{Chatbot is only end-user oriented}. We (data scientists) need something \textbf{intermediary}... when I go to the manager, he needs the insight only. He doesn't want that full narrative." (P8, Data scientist)
\end{quote}

This quote addresses the divergent needs within the data analysis workflow. Data scientists require intermediary results and detailed analysis paths, which the current multi-threaded visualization provides but a chatbot might not. Conversely, their managers often need only concise, final insights, which could potentially be fulfilled by a chatbot interface. Other participants expressed interests for the inclusion of a chatbot, seeing potential benefits for enhancing the depth of exploration:

\begin{quote}
``I'd like a chatbot. I think it would be nice to be able to talk to the hypothesis as if you were talking to \textbf{someone defending that hypothesis}, because I [..] feel like that's what people do." (P2, Developer, Figure \ref{fig:node-count-by-level})
\end{quote}

\begin{quote}
``Yeah, actually chatting about a hypothesis. Like let's say I get to hear and I wanted to try discussing it. \textbf{Like a debater} at this point that I could then [be] either for or against." (P10, Developer)
\end{quote}

% \subsubsection{Potential Improvements}
% While the ordered node-link diagram was generally well-received, participants suggested several potential improvements:

% \begin{enumerate}
% \item Offering stronger user control over hypothesis exploration, such as the ability to iterate on a single hypothesis or generate more than three hypotheses at a time.
% \item Allowing direct manipulation of dataset columns to generate hypotheses.
% \item Connecting or combining relevant hypotheses and highlighting differences between nodes about the same variables.
% \item Showing branches from one node with different user inputs and labeling each node with user inputs.
% \end{enumerate}

\subsection{Design Goal 3: Enable Integrated Engagement with Relevant Data while Exploring Hypotheses}

% \subsection{AI-generated Multimodal Information Hints for Deciding Analysis Pathway}

% The interview results also showed that the AI-generated multimodal information hints played an important role in guiding users to decide on analysis pathways to pursue during hypothesis exploration. This section explores how visual hypotheses served as affirming hints and how the blending of hypotheses and charts reduced context switching effort.

\subsubsection{Visual Hypotheses Enable Judgment of Hypothesis Grounding in Data}
Participants found that the visual hypotheses generated by the system suggested whether there were evidences of their ideas or not. This visual representation helped transform abstract thoughts into data-backed concepts. P4 and P8 described this benefit:

\begin{quote}
``I will say that the visualization of the census data was helpful in \textbf{confirming} the potential income based on the higher degrees. So it was \textbf{affirming} of that. I'm further also just the visual on the working hours and how scattered that was also \textbf{affirmed}." (P4, Business technology)
\end{quote}

\begin{quote}
``It showed me data that was \textbf{reaffirming} to my hypothesis...Like it would just be like an idea of my head that would have had no backing. The fact that I saw it with data is like OK, now this has more credibility. I'm more willing to follow it than I would have if I had just thought of it." (P8, Data scientist)
\end{quote}

The direct nature of visual hypotheses was particularly appreciated. As one researcher (P1) noted, ``I guess most useful part is the figure like the visualization...hypothesis, it's kind of indirect." This sentiment was echoed by a data scientist (P19):

\begin{quote}
``I think it's really really useful because at the end the line charts, the line graph, \textbf{it's really useful to have like a graph that shows or that is directly associated with the hypothesis} that you are seeing...I think having the charts in here, it's really really useful, to really understand what is happening, to be sure that the hypothesis that you are proposing is tied to a graph"
\end{quote}

\subsubsection{Blending Hypotheses and Charts}
An advantage of the multimodality was the seamless integration of hypotheses and visualizations. This feature reduced the effort associated with context switching between hypothesis formulation and chart creation. A data scientist (P8) enthusiastically described this benefit:

\begin{quote}
``It helps me very much and then really we love it. Really. I love it. I can say definitely it helps. The chart and the narrative. And then I get immediately and instantly, which can be transferred visualization I can say because usually we struggle with the visualization and the content when GenAI gives both. It's really easier for us."
\end{quote}

The efficiency gained from this blended approach was widely appreciated. Another data scientist (P19) noted:

\begin{quote}
``I will say that it's really easy to get hypothesis and get like charts that support the hypothesis really quick. So that's an easy way to maybe start exploring data and see what the data has, and go through there, and start like going a little bit more specific."
\end{quote}

% \subsubsection{Providing Supporting Text}
% The inclusion of supporting text as part of the multimodal information hints provided context for users. This feature helped users understand the novelty and relevance of their hypotheses within the broader research landscape. P11 (developer) explained:

% \begin{quote}
% ``It does kind of let you know someone else has come for or done that idea. Like if one we're doing trying to make their own research on something novel, then knowing, you know, at least a quick hey, has someone already tried this or not could help you. Try to test something further or no, maybe no one's thought along this line."
% \end{quote}

% \subsubsection{Potential Improvements}

% While the multimodal information hints were generally well-received, participants suggested several potential improvements. These included providing sources for preliminary results (such as code) and related work (like citations and external links) to enhance the explainability of the outputs. Additionally, participants proposed converting the hypothesis, preliminary results, and related work into preliminary presentation drafts such as slides, which could potentially make the information more accessible and easier to digest.

==> cutting-room-floor/prev-2-introduction.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure}
\includegraphics[width=1\textwidth]{figures/Model.png}
  \caption{Conceptual modeling of decision making space in a 2D space, similar to Chan et al. \cite{chanFormulatingFixatingEffects2024}. (a) (b) (c) represent the same space. (a) represents of the space of possible decisions, showing areas of superficiality and fixation relative to human intent, with the ``right thing" represented with a star potentially lying outside these areas. (b) AI-generated comprehensive exploration of all possible decisions, illustrating maximum breadth and depth. (c) A human-AI shared representation of decisions, balancing parallel exploration with iteration to efficiently navigate the decision making space.}
  \Description{}
  \label{fig:model}
\end{figure}

Data analysis workflows can be divided into two main components: ``doing the right thing" and ``doing things right." The former involves deciding on analysis directions and objects such as formulating interesting and testable hypotheses \cite{junRTisaneExternalizingConceptual2024,junHypothesisFormalizationEmpirical2022}, which are highly dependent on domain knowledge and context. The latter includes tasks such as data cleaning and refining visualizations, which are similar across different domains and contexts. Guidelines and practices for ``doing things right" in data analysis are widely accessible online, as these fundamental tasks are largely consistent across fields. As Generative AI models continue to advance, we now have a growing number of intelligent systems and agents that can assimilate guidelines and execute analysis tasks and substeps with minimal to no human supervision \cite{xieWaitGPTMonitoringSteering2024,dibiaLIDAToolAutomatic2023,tianChartGPTLeveragingLLMs2024}.

However, ``doing the right thing" – making context-appropriate decisions – remains a significant hurdle for fully autonomous systems. This capability requires a nuanced understanding of both appropriate and inappropriate decisions, including potential failure modes. While such knowledge is pervasive in human society, it often exists in tacit forms, undocumented and unpublished \cite{ackermanSharingKnowledgeExpertise2013,cetinaEpistemicCulturesHow1999,rittbergEpistemicInjusticeMathematics2018}. Human experts typically internalize these complex right-wrong classifiers within their cognitive frameworks, making it difficult to transfer this decision-making ability to artificial systems.

Even for human experts, making context-appropriate decisions is also challenging due to two main factors: superficiality (lack of depth) \cite{kahneman2011thinking} and fixation (lack of breadth) \cite{chanFormulatingFixatingEffects2024,janssonDesignFixation1991}. We can model the space of possible decisions in a 2D space, similar to the approach taken by Chan et al. \cite{chanFormulatingFixatingEffects2024}, as shown in Figure \ref{fig:model}(a). In this model, the area closer to human intent potentially represents superficiality, while the area perpendicular to human intents may indicate fixation. The ``right thing", represented by a star, might exist outside these areas. To find the ``right thing," we need iteration to increase depth and overcome superficiality, and parallel exploration to increase breadth and overcome fixation.

As the total time budget is often limited, spending more time on breadth-oriented parallel exploration reduces the time available for depth-oriented iteration. Generative AI can support both parallel exploration and iteration by harnessing its world knowledge and generative capabilities to produce potential correct pathways. Humans can then use their domain-specific knowledge and decision-making abilities to select analytical pathways to pursue. To achieve this, a shared representation between humans and AI needs to be created, balancing parallel exploration and iteration.

While using GenAI to generate all possibilities could maximize both exploration and iterations as shown in Figure \ref{fig:model}(b), this approach would produce too much information for humans to consume effectively. Instead, we propose providing information hints to help people pause or stop unpromising trajectories, thus guiding the parallel exploration and iteration process as Figure \ref{fig:model}(c).

The content of the shared representation is important for enhancing parallel exploration and iteration. Hypotheses, as high-level content in data analysis, could serve as a medium for shared representation. Using hypotheses as indicators of analytical directions or pathways offers an advantage: their inherently sketchy nature can mitigate cognitive fixation in users, promoting more flexible and creative analytical approaches. As previously discussed, to help people more flexibly explore and iterate hypotheses instead of generating and consuming all possible hypotheses, we can provide relevant information hints for each hypothesis, such as visualizations and pertinent prior research corresponding to the hypothesis to guide the exploration and iteration process.

These design considerations prompt us to ask the research question: \textbf{How can we design effective shared representations for hypothesis exploration supporting both breadth-oriented parallel exploration and depth-oriented iteration?} Our research addresses this question through the following contributions:

\begin{itemize}
    \item \textbf{System design}: we developed a GenAI-assisted hypothesis exploration tool. This tool interprets users' analytical intents, generates potential hypotheses and corresponding visual hypotheses, and retrieves relevant literature as supporting texts.
    \item \textbf{Empirical results}: the findings from a design probe (n=22) suggest that the tool could assist hypothesis exploration by providing node-link diagrams as exploration and iteration structures, and information hints, especially visual hypotheses, to guide analysis decisions.
\end{itemize}

==> cutting-room-floor/prev-discussion_conclusion.tex <==
\section{Discussion}

\subsection{Interpretation of Results}

\subsection{Beyond Hypothesis Exploration: Towards Intent-based User Interface}

The emergence of Generative AI, particularly the advanced natural language processing capabilities of Large Language Models (LLMs), potentially marks the first significant paradigm shift in user interface in 60 years \cite{nielsen2023ai}. This shift transitions from command-based interaction to intent-based outcome specification. On command-based interfaces, users need to simultaneously focus on two aspects: ``doing the right thing" by formulating the correct intent, and ``doing things right" by executing the appropriate commands, whether through command-line interfaces or graphical user interfaces. In contrast, the intent-based interaction paradigm aims to alleviate the cognitive load associated with command execution, allowing users to concentrate primarily on formulating the right intents.

Advancing GUI \cite{dingAdvancingGUIGenerative2024} to intent-based user interface \cite{dingIntentbasedUserInterfaces2024}, for coding \cite{zhangFrontendDiffusionExploring2024}

% Data analysis is an important application domain for intent-based interaction: traditionally, data analysts have to invest considerable time in command-level actions, including data cleaning, statistical testing, and modeling. The emergence of LLMs demonstrates potential in automating these processes \cite{dibiaLIDAToolAutomatic2023}, effectively ``doing things right." This automation could enable analysts to redirect their focus towards ``doing the right thing" -- namely identifying appropriate analytical directions. However, current GenAI-powered data analysis tools typically employ a bottom-up system design approach, such as developing systems translating natural language commands into visualizations \cite{dibiaLIDAToolAutomatic2023,vaithilingamDynaVisDynamicallySynthesized2024}. In contrast, a top-down method that attempts to decompose users' high-level intents remains largely unexplored. To investigate the potential of intent-based interaction in data analysis, we have chosen to focus on hypothesis exploration as the primary task for implementing and evaluating intent-based interaction paradigms.

Planning: decision making e.g. trip planning

Execution: complex and independent tasks e.g. video production

\section{Conclusion}

% anonymity check
% \begin{acks}

% \end{acks}

%% The next two lines define the bibliography style to be used, and
%% the bibliography file.
\bibliographystyle{ACM-Reference-Format}
\bibliography{sample-base}

%%
%% If your work has an appendix, this is the place to put it.

\newpage

\appendix

\section{Appendix A: Backtrack Behaviors}
\label{appendix:A}

\begin{figure}[h]
\includegraphics[width=0.8\textwidth]{figures/P3.png}
  \caption{User journey of P3 (17 backtracks in total).}
  \Description{}
  \label{fig:P3}
\end{figure}

\begin{table}[h]
    \centering
    \begin{tabular}{|c|p{4.5cm}|p{3.5cm}|p{2.2cm}|p{1.5cm}|}
        \hline
        ID & High Level Backtrack and Generate & High Level Backtrack Only & Other Backtrack & Total \\
        \hline
        Mean (Variance) & 0.91 (1.52) & 1.64 (2.15) & 1.41 (5.49) & 3.95 (12.90) \\
        \hline
        P1 & 0 & 2 & 0 & 2 \\
        \hline
        P2 & 0 & 3 & 3 & 6 \\
        \hline
        P3 & 5 & 1 & 11 & 17 \\
        \hline
        P4 & 1 & 3 & 2 & 6 \\
        \hline
        P5 & 1 & 3 & 1 & 5 \\
        \hline
        P6 & 0 & 3 & 0 & 3 \\
        \hline
        P7 & 1 & 3 & 1 & 5 \\
        \hline
        P8 & 2 & 1 & 1 & 4 \\
        \hline
        P9 & 3 & 0 & 2 & 5 \\
        \hline
        P10 & 0 & 1 & 1 & 2 \\
        \hline
        P11 & 1 & 0 & 0 & 1 \\
        \hline
        P12 & 1 & 1 & 0 & 2 \\
        \hline
        P13 & 0 & 1 & 0 & 1 \\
\hline
P14 & 0 & 0 & 0 & 0 \\
\hline
P15 & 2 & 0 & 2 & 4 \\
\hline
P16 & 1 & 1 & 1 & 3 \\
\hline
P17 & 0 & 4 & 2 & 6 \\
\hline
P18 & 0 & 5 & 2 & 7 \\
\hline
P19 & 0 & 2 & 0 & 2 \\
\hline
P20 & 0 & 0 & 0 & 0 \\
\hline
P21 & 1 & 2 & 2 & 5 \\
\hline
P22 & 1 & 0 & 0 & 1 \\
\hline
    \end{tabular}
    \caption{Backtrack behaviors: check a node which is not on the path from the root node or does not have the same parent node.}
    \label{tab:backtrack}
\end{table}

\clearpage

\section{Appendix B: Table of User Engagement with Visual Hypotheses}
\label{appendix:B}

\begin{table}[h]
    \centering
    \begin{tabular}{|c|p{4cm}|p{4.5cm}|p{1.5cm}|}
        \hline
        ID & Initial expansion of visual hypotheses & Re-expansion of visual hypotheses & Total \\
        \hline
        Mean (Variance) & 6.32 (4.90)  & 1.91 (3.85) & 8.23 (7.41) \\
        \hline
        P1 & 18 & 5 & 23 \\
        \hline
        P2 & 5 & 4 & 9 \\
        \hline
        P3 & 13 & 3 & 16 \\
        \hline
        P4 & 9 & 1 & 10 \\
        \hline
        P5 & 9 & 2 & 11 \\
        \hline
        P6 & 5 & 1 & 6 \\
        \hline
        P7 & 7 & 2 & 9 \\
        \hline
        P8 & 8 & 2 & 10 \\
        \hline
        P9 & 2 & 0 & 2 \\
        \hline
        P10 & 11 & 0 & 11 \\
        \hline
        P11 & 14 & 1 & 15 \\
        \hline
        P12 & 1 & 1 & 2 \\
        \hline
        P13 & 0 & 0 & 0 \\
\hline
P14 & 2 & 0 & 2 \\
\hline
P15 & 2 & 0 & 2 \\
\hline
P16 & 3 & 0 & 3 \\
\hline
P17 & 2 & 0 & 2 \\
\hline
P18 & 6 & 1 & 7 \\
\hline
P19 & 11 & 18 & 29 \\
\hline
P20 & 4 & 1 & 5 \\
\hline
P21 & 0 & 0 & 0 \\
\hline
P22 & 7 & 0 & 7 \\
\hline
    \end{tabular}
    \caption{User engagement with visual hypotheses.}
    \label{tab:backtrack}
\end{table}

==> cutting-room-floor/prev-introduction.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure}
\includegraphics[width=1\textwidth]{figures/Model.png}
  \caption{Why we need guardrail for exploration.}
  \Description{}
  \label{fig:model}
\end{figure}

Existing data analysis workflows have predominantly focused on ``doing things right" such as data cleaning and refining visualizations. Consequently, guidelines, practices and tools for conducting basic data analysis tasks correctly are widely accessible online. As the capabilities of generative AI systems continue to advance, autonomous systems can assimilate such guidelines and execute those fundamental data analysis tasks with minimal human supervision \cite{dibiaLIDAToolAutomatic2023}.

However, engaging in high-level, intent-based planning—often referred to as ``doing the right thing"—such as formulating testable and interesting hypotheses, remains a challenge for fully autonomous systems, as it requires discerning appropriate actions through a nuanced understanding of inappropriate approaches, including failures. Such knowledge is ubiquitous in human society but often remains undocumented or unpublished \cite{ackermanSharingKnowledgeExpertise2013,cetinaEpistemicCulturesHow1999,rittbergEpistemicInjusticeMathematics2018}, which makes those right-wrong classifiers typically reside within the cognitive frameworks of human experts.

% Moreover, recent research has demonstrated the potential for generative AI to operate at the ideation and planning level, such as generating research ideas \cite{siCanLLMsGenerate2024} and creating analogies \cite{dingFluidTransformersCreative2023}.

Therefore, a collaborative approach between humans and AI is essential to explore and determine the correct course of action in various analytical contexts. This partnership leverages the complementary strengths of human expertise and AI capabilities to navigate the complexities of decision-making processes in data analysis, particularly in areas where the distinction between right and wrong approaches is subtle and context-dependent.

To facilitate this high-level human-AI collaboration, it is important to design a shared representation wherein AI systems can harness their world knowledge and generative capabilities to produce potential correct pathways, while humans can use their domain-specific knowledge and decision-making abilities to select analytical pathway to pursue. Hypotheses exploration, as a high-level task in data analysis, could serve as a promising context for implementing and evaluating that collaborative framework. The utilization of hypotheses as content within the shared representation, serving as indicators of analytical pathways, offers an advantage: the inherently sketchy nature of hypotheses can mitigate cognitive fixation in users, thereby promoting more flexible and creative analytical approaches.

To further reduce fixation and promote exploration, we can apply the concept of parallel prototyping \cite{dowParallelPrototypingLeads2010} by generating multiple hypotheses simultaneously, allowing humans to select which ones to investigate and refine further. It's important to recognize that hypothesis selection is inherently context-dependent, and a text-based hypothesis alone is insufficient. An effective hypothesis exploration tool needs to provide relevant information hints, including data-driven visualizations and pertinent prior research to guide the selection process. Those design considerations prompt us to ask the research question: \textbf{How can we design effective shared representations for human-AI collaboration in hypothesis exploration?} Our research addresses this research questions through the following contributions:

\begin{itemize}
    \item System design: To facilitate high-level human-AI collaboration in data analysis, we conducted a series of formative studies and developed a GenAI-assisted hypothesis exploration tool. This tool interprets users' analytical intents, generates potential hypotheses, provides preliminary visualizations, and retrieves relevant literature. 
    \item Empirical study: We conducted a design probe study (n=22) to investigate how this intent-based tool might guide users toward valuable analytical directions. Our findings suggest that the tool could enhance data analysis by enabling users to focus on higher-level decision-making and explore diverse analytical pathways.
\end{itemize}

% Our primary research goal is to effectively design GenAI-assisted hypothesis exploration. To approach this task, we've broken it down into two research questions:

% \begin{itemize}
%     \item \textbf{RQ1:} How to present multiple hypotheses to support hypothesis exploration and iteration? 
%     \item \textbf{RQ2:} What form or structure should each hypothesis take (in order to explore hypothesis, whether to proceed)?
% \end{itemize}



% Hence, we propose two research question:

% \begin{itemize}
%     \item \RQO
%     \item \RQT
% \end{itemize}

==> cutting-room-floor/prev-results.tex <==
\section{Results}
\label{sec:results}

\begin{figure}[h]
\includegraphics[width=1\textwidth]{figures/workflow.png}
  \caption{Walk-through of hypothesis exploration functions and user journey of P5.}
  \Description{}
  \label{fig:user-journey}
\end{figure}

\subsection{Results Overview}

Participants' overall attitude towards the hypothesis exploration tool was positive, as evidenced by responses to Q5 in our semi-structured interview: ``After using this tool, do you want to use GenAI tools for hypothesis formulation in the future?" A majority (82\%) expressed enthusiasm, exemplified by P12's statement: ``I absolutely would use this, 100\%." One participant (9\%) showed selective interest, expressing openness to the tool's data visualization capabilities while reserving judgment on its use for hypothesis formulation. The final participant (9\%) cited a commitment to originality and privacy concerns: ``I'm trying to make something novel myself. I don't want to have to cite it or accidentally give away one of my ideas." To illustrate how participants actually engaged with the hypothesis exploration tool, Figure \ref{fig:user-journey} provides a walk-through of P5's study process. Below are three exemplary GenAI-generated hypotheses that participants bookmarked:

\begin{itemize}
    \item \textbf{Age Effect}: There is a variance in income between married and non-married individuals within different age groups. (P1)
    \item \textbf{Occupation Type}: There is a significant difference in income levels based on occupation types between married and unmarried individuals. (P2)
    \item \textbf{Gender Impact}: There is a significant correlation between holding an advanced degree and higher incomes with the additional factor of gender, affecting married individuals differently compared to unmarried individuals. (P2)
    \item \textbf{Investment Growth}: Higher income earners exhibit a faster growth rate of their financial assets over time. (P5)
\end{itemize}

\begin{figure}
\includegraphics[width=1\textwidth]{figures/Node-count.png}
  \caption{Count of nodes by level, starting from level 2 given that level 0 always has 1 analysis intent node and level 1 always has 5 initial hypothesis nodes. As the depth increases, the count of nodes per level progressively decreases, reflecting a more focused analysis at deeper levels of the tree structure.}
  \Description{}
  \label{fig:node-count-by-level}
\end{figure}

% \begin{figure}
% \centering
% \begin{subfigure}[b]{0.48\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{figures/BD.png}
%     \caption{Maxmium breadth and depth of node-link diagrams.}
%     \label{fig:BD}
% \end{subfigure}
% \hfill
% \begin{subfigure}[b]{0.48\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{figures/CountByLevel.png}
%     \caption{Counts of nodes by levels.}
%     \label{fig:Level}
% \end{subfigure}
% \caption{Analysis of node-link diagrams created by participants: (a) Maximum breadth (maximum count of nodes on a level) and maximum depth (maximum count of levels), (b) Count of nodes by level, starting from level 2 given that level 0 always has 1 analysis intent node and level 1 always has 5 initial hypothesis nodes.}
% \Description{Two scatter plots side by side. The left plot shows the maximum breadth vs depth of node-link diagrams. The right plot shows the count of nodes at different levels of the diagrams.}
% \label{fig:combined}
% \end{figure} 

% Figure \ref{fig:combined} shows the analysis of the node-link diagram structure, illustrating the overall diagram patterns through the distribution of maximum breadth and depth in Figure \ref{fig:BD}, and individual exploration patterns via the counts of nodes by levels in Figure \ref{fig:Level}. Four participants (P2, P5, P20, P13) reached level 6 which was the maximum depth supported by the screen size.

While participants might not have explored every node on their diagrams. To account for this, we analyzed user interactions by tracking the number of nodes explored, as shown in Figure \ref{fig:nodes-count}. We also examined user engagement with the GenAI-generated visualizations corresponding to each hypothesis. Figure \ref{fig:engage-hist} illustrates whether and how often participants (re-)expanded these visual hypotheses.

\begin{figure}
\includegraphics[width=1\textwidth]{figures/Counts.png}
  \caption{Counts of total number of nodes explored (number of nodes clicked + number of new hypothesis branch generated, a new node will be displayed when a new branch is generated), number of nodes clicked, number of new hypothesis branch generated.}
  \Description{}
  \label{fig:nodes-count}
\end{figure}

\begin{figure}
\includegraphics[width=1\textwidth]{figures/Engage.png}
  \caption{Histograms depicting user engagement with visual hypotheses. The data illustrates two types of interactions: initial expansion (opening a visual hypothesis for the first time) and re-expansion (reopening a previously viewed visual hypothesis). Light blue bars represent participants who did not (re-)expand any visual hypothesis.}
  \Description{}
  \label{fig:engage-hist}
\end{figure}

The sequence of user interactions formed complex exploration patterns, exemplified by the detailed user journey of P3 (see Figure \ref{fig:P3} in Appendix \ref{appendix:A}). P3's hypothesis exploration process with 17 instances of backtracking highlights the prevalence of such behaviors in the exploration process in the node-link diagram. It prompted a more in-depth analysis of this phenomenon across all participants. Figure \ref{fig:backtrack-hist} illustrates the various types of backtracking behaviors: high level backtrack and generate, high level backtrack only, and other backtrack.

4 participants re-generated to replace previous branches once (3 not backtrack, 1 other backtrack)

\begin{figure}
\includegraphics[width=0.6\textwidth]{figures/Backtrack.png}
  \caption{Histograms depicting backtrack behaviors: backtracking previously created branches. The data illustrates three types of backtrack behaviors: high level backtrack and generate (revisit a hypothesis node on a higher level and not on the trajectory from the current node to the root node, and generate new branch from the node), high level backtrack only (only revisit a hypothesis node on a high level and not on the current trajectory) and other backtrack (revisit a hypothesis node but not on a higher level).}
  \Description{}
  \label{fig:backtrack-hist}
\end{figure}

\subsection{Ordered Node-link Diagram as Shared Representation of Analysis Pathways}

\subsubsection{Rapidly prototype and test alternative hypotheses in multi-threads}

\begin{quote}
    ``What I thought it was really cool is every time you've done your piece of analysis, as you go to your supervisor and you say, `Look, this is what I found.' 'Ohh that's really interesting. I wonder if you looked at it this way', but you never have time to do that…So from that point of view, I think it's really good for those additional hypothesis that you might want to go in and test." (P12, UX researcher)
\end{quote}

\begin{quote}
    ``When you propose a new hypothesis, it does not give you only one option. It gives you more than one, so you can start like exploring other branches and so that was really helpful." (P19, Data scientist)
\end{quote}

\begin{quote}
    ``It gives me the options instead of me thinking of it. It gives me the \textbf{multiple options} based on my hypothesis. What I am thinking of right? So that dimension it is giving it for the next level of hypothesis. I want to create it, so that is what the tool is helping us. That is the best part of it. So once I finalize job rule right, then the successive hypothesis, when it creates it gives 3 dimensions right? So one is different dimensions, that is what it is helping us." (P13, Consultant)
\end{quote}

avoid fixation / bias

\begin{quote}
    ``And I think as well, like researchers tend to get, tend to get dug in with particular variables, say like if you're if genders on your mind, they'll think of gender, but maybe it won't cross their mind to look at marital status. But when it's there in front of you, you're gonna `Ohh yeah, why don't I think? Let's have a look at that as well'." (P12, UX researcher)
\end{quote}

\begin{quote}
``I think it is a very useful tool that would help kind of take away bias to a certain extent. I feel like we have a lot of bias or too much personal views that can kind of formulate hypothesis." (P3, Global sales)
\end{quote}

\begin{quote}
``There was probably prior biases…if you were to ask me like without having seen any of this tool, what do you think correlates to higher income? I probably could have told you years of experience and like number of the degrees." (P4, Business technology)
\end{quote}

\subsubsection{Tree diagram as guardrails, limiting users' imagination}

\begin{quote}
``The tree diagram is like guardrails I would say yes it does (help me), because it \textbf{limits my imagination down to kind of selectable options}. So it puts boundaries on my creativity will still allowing me to, like, follow different paths I might have, that I might come up with.
So like guardrails I guess would probably be the best way to sum it up. The guardrails it imposes focuses me. 
" (P10, Developer)
\end{quote}

P10 actually only drilled down, with only one branch

\subsubsection{Clear workflow to drill down}

focus on one thread

\begin{quote}
    ``I think it's really helpful because it puts like the hypothesis into \textbf{buckets}. So you know that you will have a hypothesis for location level, a hypothesis for the work hours. And at the end, I think that this advantage of that tree diagram could be that \textbf{you only focus on one topic and forget about the rest}." (P19, Data scientist)
\end{quote}

drill down

\begin{quote}
    ``It is really helpful in connecting from one hypothesis to another hypothesis until it achieves my goal, right? That is the best part of tree diagram, that helped me to \textbf{drive through each and every hypothesis at each level and drill down to my goal}. That is what the best part of this tree, this \textbf{hypothesis model}." (P13, Consultant)
\end{quote}

logic flow, easy to follow

\begin{quote}
    ``It just gives you a \textbf{logical flow} to like, which variables belong in which. It's like a visualization of where variables are belong, where they're clustered. Yeah, it just means you go through it very quickly." (P12, UX researcher)
\end{quote}

\begin{quote}
    ``It allows you to figure out how things are connected. I thought it was \textbf{pretty easy to read and follow}. This helps me understand the data set by helping me understand what different hypothesis were connected and how under like what topic." (P3, Global sales)
\end{quote}

like that the selected branch is spread out

\begin{quote}
``I mean its user interface is super easy to use. I mean you can click and explore. Uh, and I feel like it's very easy to read because \textbf{the options are spread out enough}. I mean, as the tree gets further down, it gets more specific. So that I like that." (P5, Developer)
\end{quote}

\subsubsection{Provide overview, support backtracking}

backtrack: recreate, recheck, reread

backtrack is one way to increase the breadth

\begin{quote}
    ``This visualization tree, it's like organized hierarchy way. It was a structured and where we can easily get to know like, if we miss it somewhere, for example, in the educational level option, if you miss somewhere then to \textbf{recreate} and to \textbf{reread} it. So that time, this hierarchy level tree structure visualization helps us to \textbf{check again}, \textbf{recheck and analyze it}." (P18, Consultant)
\end{quote}

P18 had multiple branches, under educational level, work hours, occupation

which area it is more focused

\begin{quote}
``It helps to determine \textbf{which area it is more focused}, like which area it is affecting, like for what is the main reason of in income inequality and education level, in which area of education level it's more affecting. What is the main cause of income inequality?" (P9, Developer)
\end{quote}

\subsubsection{Potential improvements on shared representation}

Connecting or combining relevant hypotheses, highlighting difference between nodes about same variables

Showing branches from one node with different user inputs, labeling each node with user inputs

Converting the hypothesis, preliminary results and related work into slides

\subsection{GenAI-generated Multimodal Information Hints for Deciding Analysis Pathway}

\subsubsection{Visual hypotheses as hints to affirm their hypotheses}

visual hypotheses as hints, sketch

\begin{quote}
``It showed me data that was \textbf{reaffirming} to my hypothesis...Like it would just be like an idea of my head that would have had no backing. The fact that I saw it with data is like OK, now this has more credibility. I'm more willing to follow it than I would have if I had just thought of it." (P8, Data scientist)
\end{quote}

\begin{quote}
``I will say that the visualization of the census data was helpful in \textbf{confirming} the potential income based on the higher degrees. So it was affirming of that. I'm further also just the visual on the working hours and how scattered that was also affirmed." (P4, Business technology)
\end{quote}

The visual hypothesis is more direct than the text hypothesis: ``I guess most useful part is the figure like the visualization...hypothesis, it's kind of \textbf{indirect}." (P1, researcher)

\begin{quote}
``I think it's really really useful because at the end the line charts, the line graph, it's really useful to have like a graph that shows or that is \textbf{directly associated with the hypothesis} that you are seeing...I think the having the charts in here, it's really really useful, to really understand what is happening, to be sure that the hypothesis that you are proposing is tied to a graph" (P19, Data scientist)
\end{quote}

\subsubsection{Blending hypotheses and charts}

Reduce the workload of context switching between formulating hypothesis and creating visualizations

\begin{quote}
``It helps me very much and then really we love it. Really. I love it. I can say definitely it helps. The chart and the narrative. And then I get immediately and instantly, which can be transferred visualization I can say because usually we struggle with the visualization and the content when GenAI gives both. It's really easier for us. That the visualization, visualization is the first point and then comes to the narrative. I mean the content."

``It's really very, very nice. I can tell you I loved it. Because I'm I copy pasting something 10 charts for the different things...It reduces lot of things. Just taking chart and then chart is already prepared and already narratives has been written. Yes too cool." 

``If I get this tool, I'll prefer this tool with the chart and the narrative. I was really looking for the combination of data analysis and the data visualization along with some kind of a content making. Only content making will not help me."

(P8, Data scientist)
\end{quote}

\begin{quote}
``I will say that it's really easy to get hypothesis and get like charts that support the hypothesis really quick. So that's an easy way to maybe start exploring data and see what the data has, and go through there, and start like going a little bit more specific. So yeah, I will say that it's quick, and you get hypothesis and charts that support that hypothesis really quick." (P19, Data scientist)
\end{quote}

\subsubsection{Providing supporting text}

\begin{quote}
``It does kind of let you know someone else has come for or done that idea. Like if one we're doing trying to make their own research on something novel, then knowing, you know, at least a quick hey, has someone already tried this or not could help you. Try to test something further or no, maybe no one's thought along this line." (P11, Developer)
\end{quote}

\subsubsection{Potential improvements on generating multimodal information hints}

Offering stronger user control on the hypothesis exploration with user input:
iterating on only one hypothesis or generate more than three hypotheses
directly manipulating the columns of the dataset to generate hypothesis

Sources of preliminary results (code) and related work (citations, external links), make the outputs more explainable
